Robustness to Transformations Across Categories: Is Robustness To Transformations Driven by Invariant Neural Representations?

Deep Convolutional Neural Networks (DCNNs) have demonstrated impressive robustness to recognize objects under transformations (eg. blur or noise) when these transformations are included in the training set. A hypothesis to explain such robustness is that DCNNs develop invariant neural representations that remain unaltered when the image is transformed. However, to what extent this hypothesis holds true is an outstanding question, as robustness to transformations could be achieved with properties different from invariance, eg. parts of the network could be specialized to recognize either transformed or non-transformed images. This paper investigates the conditions under which invariant neural representations emerge by leveraging that they facilitate robustness to transformations beyond the training distribution. Concretely, we analyze a training paradigm in which only some object categories are seen transformed during training and evaluate whether the DCNN is robust to transformations across categories not seen transformed. Our results with state-of-the-art DCNNs indicate that invariant neural representations do not always drive robustness to transformations, as networks show robustness for categories seen transformed during training even in the absence of invariant neural representations. Invariance only emerges as the number of transformed categories in the training set is increased. This phenomenon is much more prominent with local transformations such as blurring and high-pass filtering than geometric transformations such as rotation and thinning, which entail changes in the spatial arrangement of the object. Our results contribute to a better understanding of invariant neural representations in deep learning and the conditions under which it spontaneously emerges.

==> category.tex <==
\section{Results: Category Dependence of the Robustness to Transformations}



==> figs/Figure3-alt.tex <==

\begin{figure*}[t!]
\centering
\scriptsize
\includegraphics[width=\textwidth]{figs/complete_paper_figures/Figure3-alt.pdf}
\caption{\emph{Active Neurons and Invariance when all categories are \emph{seen-transformed}.} (a) Distribution of the number of active neurons per image and the number of images that activate a neuron. (b) and (c) Violin plots of the invariance coefficient among neurons in the penultimate layer, for FaceScrub and ImageNet, respectively. The invariance to each transformation is shown for  networks trained with the transformation applied to all categories (indicated with $x + T(x)$) and for networks trained only with non-transformed images ($x$). }
\label{fig:fig3}
\vspace{1cm}
\end{figure*}


==> figs/Imagenet_invariance_accuracy.tex <==

\begin{figure*}[t!]
\centering
\scriptsize
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.25\textwidth]{figs/paper_plots/Imagenet_Testing_Accuracy_convol_seen_transformed_figure.pdf} &
\includegraphics[width=0.25\textwidth]{figs/paper_plots/Imagenet_Testing_Accuracy_convol_unseen_transformed_figure.pdf} \\
 (a) & (b)\\[{0.15cm}]
\includegraphics[width=0.25\textwidth]{figs/paper_plots/Imagenet_Invariance_convol_seen_transformed_figure.pdf} &
\includegraphics[width=0.25\textwidth]{figs/paper_plots/Imagenet_Invariance_convol_unseen_transformed_figure.pdf} \\
 (c) & (d) \\[{0.15cm}]
\includegraphics[width=0.25\textwidth]{figs/paper_plots/Imagenet_Accuracy_Invariance_Scatter_convol_seen_transformed_figure.pdf} &
\includegraphics[width=0.25\textwidth]{figs/paper_plots/Imagenet_Accuracy_Invariance_Scatter_convol_unseen_transformed_figure.pdf} \\
(e) & (f) \\[{0.15cm}]
\end{tabular}
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:imagenet_invariance}
\end{figure*}



==> figs/Imagenet_violin_plots.tex <==

\begin{figure*}[t!]
\centering
\scriptsize
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.5\textwidth]{figs/paper_plots/Imagenet_Invariance_Distribution_high_pass.pdf} \\
 (a)  \\[{0.15cm}]
\includegraphics[width=0.5\textwidth]{figs/paper_plots/Imagenet_Invariance_Distribution_low_pass.pdf} \\
(b) \\[{0.15cm}]
\includegraphics[width=0.5\textwidth]{figs/paper_plots/Imagenet_Invariance_Distribution_noise.pdf} \\
(c) \\[{0.15cm}]
\end{tabular}
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:imagenet_violins}
\end{figure*}



==> figs/categories.tex <==

\begin{figure*}[t!]
\centering
\scriptsize
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.25\textwidth]{figs/categories/color.pdf} &
\includegraphics[width=0.25\textwidth]{figs/categories/filter.pdf} &
\includegraphics[width=0.25\textwidth]{figs/categories/noise.pdf} &
\includegraphics[width=0.25\textwidth]{figs/categories/geometry.pdf} \\
 (a) & (b) & (c) & (d) \\[{0.15cm}]
\includegraphics[width=0.25\textwidth]{figs/categories/trans_color.pdf} &
\includegraphics[width=0.25\textwidth]{figs/categories/trans_filter.pdf} &
\includegraphics[width=0.25\textwidth]{figs/categories/trans_noise.pdf} &
\includegraphics[width=0.25\textwidth]{figs/categories/trans_geometry.pdf} \\
(e) & (f) & (g) & (h) \\[{0.15cm}]
\includegraphics[width=0.25\textwidth]{figs/categories/conf_color.pdf} &
\includegraphics[width=0.25\textwidth]{figs/categories/conf_filter.pdf} &
\includegraphics[width=0.25\textwidth]{figs/categories/conf_noise.pdf} &
\includegraphics[width=0.25\textwidth]{figs/categories/conf_geometry.pdf} \\
(i) & (j) & (k) & (l) \\
\end{tabular}
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:paraadigm}
\end{figure*}



==> figs/categories_mod.tex <==

\begin{figure*}[t!]
\centering
\scriptsize
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.262\textwidth]{figs/paper_plots/Testing_Accuracy_color_seen_transformed_figure.pdf} &
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Testing_Accuracy_convol_seen_transformed_figure.pdf}&
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Testing_Accuracy_noise_seen_transformed_figure.pdf} &
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Testing_Accuracy_geometry_seen_transformed_figure.pdf} \\
 (a) & (b) & (c) & (d) \\[{0.15cm}]
\includegraphics[width=0.262\textwidth]{figs/paper_plots/Testing_Accuracy_color_unseen_transformed_figure.pdf} &
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Testing_Accuracy_convol_unseen_transformed_figure.pdf}&
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Testing_Accuracy_noise_unseen_transformed_figure.pdf} &
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Testing_Accuracy_geometry_unseen_transformed_figure.pdf} \\
(e) & (f) & (g) & (h) \\[{0.15cm}]
\end{tabular}
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:categories}
\end{figure*}



==> figs/distortions.tex <==


\begin{figure}[t!]
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{\hspace{0.1cm}}c@{\hspace{0.4cm}}c@{\hspace{0.05cm}}c@{\extracolsep{0.4cm}}c@{\extracolsep{0.0cm}\hspace{0.05cm}}c@{\hspace{0.05cm}}c@{}}
 & \multicolumn{2}{c}{\bf Color Transf.} & \multicolumn{3}{c}{\bf Geometric Transf.} \\ \cline{2-3} \cline{4-6}
 \emph{None} & \emph{Gray-scale} & \emph{Color Rotation} & \emph{Thinning} & \emph{Rotate $\pi/2$} & \emph{Rotate $\pi$}   \\
\includegraphics[width=0.14\textwidth]{figs/distortions/none.jpg} &
\includegraphics[width=0.14\textwidth]{figs/distortions/grayscale.jpg} &
\includegraphics[width=0.14\textwidth]{figs/distortions/color.jpg} &
\includegraphics[width=0.14\textwidth]{figs/distortions/thinning.jpg} &
\includegraphics[width=0.14\textwidth]{figs/distortions/rotate90.jpg} &
\includegraphics[width=0.14\textwidth]{figs/distortions/rotate180.jpg} 
\vspace{0.2cm}
\end{tabular}
}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c@{\hspace{0.05cm}}c@{\hspace{0.05cm}}c@{\hspace{0.05cm}}c@{\extracolsep{0.4cm}}c@{\extracolsep{-0.0cm}\hspace{0.05cm}}c@{}}
 \multicolumn{4}{c}{\bf Convolutional Transf.} & \multicolumn{2}{c}{\bf Noise Transf.} \\ \cline{0-3} \cline{5-6}
\emph{Blur} & \emph{High Pass Filter} & \emph{Horiz. Filter} & \emph{Vert. Filter}  & \emph{Gauss. Noise} & \emph{Salt-and-Pepper} \\
\includegraphics[width=0.135\textwidth]{figs/distortions/low_pass.jpg} &
\includegraphics[width=0.135\textwidth]{figs/distortions/high_pass.jpg} &
\includegraphics[width=0.135\textwidth]{figs/distortions/horizontalfilter.jpg} &
\includegraphics[width=0.135\textwidth]{figs/distortions/verticalfilter.jpg} &
\includegraphics[width=0.135\textwidth]{figs/distortions/noise.jpg} &
\includegraphics[width=0.135\textwidth]{figs/distortions/salt_pepper.jpg} 
\end{tabular}
}
\caption{\emph{Image Transformations.} We analyze $12$ image transformations, organized in four families: color, convolutional, noise and geometric. }
\label{fig:distortions}
\vspace{-0.5cm}
\end{figure}


==> figs/faces_violin_plots.tex <==

\begin{figure*}[t!]
\centering
\scriptsize
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.5\textwidth]{figs/paper_plots/Invariance_Distribution_high_pass.pdf} \\
 (a)  \\[{0.15cm}]
\includegraphics[width=0.5\textwidth]{figs/paper_plots/Invariance_Distribution_low_pass.pdf} \\
(b) \\[{0.15cm}]
\includegraphics[width=0.5\textwidth]{figs/paper_plots/Invariance_Distribution_rotate180.pdf} \\
(c) \\[{0.15cm}]
\end{tabular}
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:face_violin}
\end{figure*}



==> figs/heatmaps.tex <==

\begin{figure}[t!]
\centering
\footnotesize
\begin{tabular}{@{}c@{}c@{}}
\includegraphics[width=0.5\textwidth]{figs/heatmaps/400.pdf} &
\includegraphics[width=0.5\textwidth]{figs/heatmaps/400.pdf} \\
(a) & (b)\\
\end{tabular}
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:heat400}
\end{figure}

==> figs/heatmaps_confusion.tex <==

\begin{figure}[t!]
\centering
\footnotesize
\begin{tabular}{@{}c@{}c@{}}
\includegraphics[width=0.5\textwidth]{figs/heatmaps/conf_350.pdf} &
\includegraphics[width=0.5\textwidth]{figs/heatmaps/conf_350.pdf} \\
(a) & (b)\\
\end{tabular}
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:heat_transfer}
\end{figure}

==> figs/heatmaps_transfer.tex <==

\begin{figure}[t!]
\centering
\footnotesize
\begin{tabular}{@{}c@{}c@{}}
\includegraphics[width=0.5\textwidth]{figs/heatmaps/trans_350.pdf} &
\includegraphics[width=0.5\textwidth]{figs/heatmaps/trans_350.pdf} \\
(a) & (b)\\
\end{tabular}
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:heat_transfer}
\end{figure}

==> figs/invariance.tex <==

\begin{figure*}[t!]
\centering
\scriptsize
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.258\textwidth]{figs/paper_plots/Invariance_color_all_figure.pdf} &
\includegraphics[width=0.242\textwidth]{figs/paper_plots/Invariance_convol_all_figure.pdf}&
\includegraphics[width=0.242\textwidth]{figs/paper_plots/Invariance_noise_all_figure.pdf} &
\includegraphics[width=0.258\textwidth]{figs/paper_plots/Invariance_geometry_all_figure.pdf} \\
 (a) & (b) & (c) & (d) \\[{0.15cm}]
\includegraphics[width=0.258\textwidth]{figs/paper_plots/Accuracy_Invariance_Scatter_color_seen_transformed_figure.pdf} &
\includegraphics[width=0.242\textwidth]{figs/paper_plots/Accuracy_Invariance_Scatter_convol_seen_transformed_figure.pdf}&
\includegraphics[width=0.242\textwidth]{figs/paper_plots/Accuracy_Invariance_Scatter_noise_seen_transformed_figure.pdf} &
\includegraphics[width=0.258\textwidth]{figs/paper_plots/Accuracy_Invariance_Scatter_geometry_seen_transformed_figure.pdf} \\
(e) & (f) & (g) & (h) \\[{0.15cm}]
\includegraphics[width=0.258\textwidth]{figs/paper_plots/Accuracy_Invariance_Scatter_color_unseen_transformed_figure.pdf} &
\includegraphics[width=0.242\textwidth]{figs/paper_plots/Accuracy_Invariance_Scatter_convol_unseen_transformed_figure.pdf}&
\includegraphics[width=0.242\textwidth]{figs/paper_plots/Accuracy_Invariance_Scatter_noise_unseen_transformed_figure.pdf} &
\includegraphics[width=0.258\textwidth]{figs/paper_plots/Accuracy_Invariance_Scatter_geometry_unseen_transformed_figure.pdf} \\
(i) & (j) & (k) & (l) \\
\end{tabular}
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:faces_invariance}
\end{figure*}









==> figs/layer_invariance.tex <==

\begin{figure*}[t!]
\centering
\scriptsize
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.262\textwidth]{figs/paper_plots/Layer_wise_Invariance_color_all_figure.pdf} &
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Layer_wise_Invariance_convol_all_figure.pdf}&
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Layer_wise_Invariance_noise_all_figure.pdf} &
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Layer_wise_Invariance_geometry_all_figure.pdf} \\
 (a) & (b) & (c) & (d) \\[{0.15cm}]
\includegraphics[width=0.262\textwidth]{figs/paper_plots/Layer_wise_Invariance_color_seen_transformed_figure.pdf} &
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Layer_wise_Invariance_convol_seen_transformed_figure.pdf}&
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Layer_wise_Invariance_noise_seen_transformed_figure.pdf} &
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Layer_wise_Invariance_geometry_seen_transformed_figure.pdf} \\
(e) & (f) & (g) & (h) \\[{0.15cm}]
\includegraphics[width=0.262\textwidth]{figs/paper_plots/Layer_wise_Invariance_color_unseen_transformed_figure.pdf} &
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Layer_wise_Invariance_convol_unseen_transformed_figure.pdf}&
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Layer_wise_Invariance_noise_unseen_transformed_figure.pdf} &
\includegraphics[width=0.246\textwidth]{figs/paper_plots/Layer_wise_Invariance_geometry_unseen_transformed_figure.pdf} \\
(i) & (j) & (k) & (l) \\
\end{tabular}
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:layer_invariance}
\end{figure*}









==> figs/paradigm.tex <==
\begin{figure}[t!]
A B
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:paradigm}
\end{figure}

==> figs/threshold_figures.tex <==

\begin{figure*}[t!]
\centering
\scriptsize
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.255\textwidth]{figs/paper_plots/Below_Threshold400-transformed_set.pdf} &
\includegraphics[width=0.245\textwidth]{figs/paper_plots/Above_Threshold400-transformed_set.pdf} \\
 (a) & (b) \\[{0.15cm}]
 \includegraphics[width=0.25\textwidth]{figs/paper_plots/Below_Threshold_Count.pdf} &
\includegraphics[width=0.25\textwidth]{figs/paper_plots/Above_Threshold_Count.pdf} \\
(c) & (d)\\[{0.15cm}]
\end{tabular}
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:faces_threshold}
\end{figure*}



==> figs/transfer_bar.tex <==

\begin{figure}[t!]
\centering
\footnotesize
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.25\textwidth]{figs/transfer_bar/color.pdf} &
\includegraphics[width=0.25\textwidth]{figs/transfer_bar/filter.pdf} &
\includegraphics[width=0.25\textwidth]{figs/transfer_bar/noise.pdf} &
\includegraphics[width=0.25\textwidth]{figs/transfer_bar/geometry.pdf} \\
(a) & (b) & (c) & (d) \\
\includegraphics[width=0.25\textwidth]{figs/transfer_bar/objects_color.pdf} &
\includegraphics[width=0.25\textwidth]{figs/transfer_bar/objects_filter.pdf} &
\includegraphics[width=0.25\textwidth]{figs/transfer_bar/objects_noise.pdf} &
\includegraphics[width=0.25\textwidth]{figs/transfer_bar/objects_geometry.pdf} \\
(e) & (f) & (g) & (h) \\
\end{tabular}
\caption{\emph{Testing Category Dependent Robustness.}  }
\label{fig:paraadigm}
\end{figure}

==> figs/transform_vs_notransform.tex <==
\begin{figure*}[t!]
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=\textwidth]{figs/paper_plots/Figure_1.pdf} \\
\end{tabular}
}
\caption{\emph{Invariance to transformation}  }
\label{fig:faces_transform_invariance}
\end{figure*}


